Towards Exemplar-Free Continual Learning in Vision Transformers: an Account of Attention, Functional and Weight Regularization

In this paper, we investigate the continual learning of Vision Transformers (ViT) for the challenging exemplar-free scenario, with special focus on how to efficiently distill the knowledge of its crucial self-attention mechanism (SAM). Our work takes an initial step towards a surgical investigation of SAM for designing coherent continual learning methods in ViTs. We first carry out an evaluation of established continual learning regularization techniques. We then examine the effect of regularization when applied to two key enablers of SAM: (a) the contextualized embedding layers, for their ability to capture well-scaled representations with respect to the values, and (b) the prescaled attention maps, for carrying value-independent global contextual information. We depict the perks of each distilling strategy on two image recognition benchmarks (CIFAR100 and ImageNet-32) -- while (a) leads to a better overall accuracy, (b) helps enhance the rigidity by maintaining competitive performances. Furthermore, we identify the limitation imposed by the symmetric nature of regularization losses. To alleviate this, we propose an asymmetric variant and apply it to the pooled output distillation (POD) loss adapted for ViTs. Our experiments confirm that introducing asymmetry to POD boosts its plasticity while retaining stability across (a) and (b). Moreover, we acknowledge low forgetting measures for all the compared methods, indicating that ViTs might be naturally inclined continual learner

==> chunks.tex <==
  a new Pool loss applicable in both attentional and functional submodules. The new loss unlocks best performances in 


In doing so we discuss the symmetric nature of the losses and devise an asymmetric counterpart showing more indulgence in plasticity achieving better


two techniques to enhance their rigidity. First, we argued that the often overlooked prescaled self-attention maps can be considered as a better choice over the contextualized embedding vectors for distilling knowledge. Our extensive experiments across CIFAR10, CIFAR100 and ImageNet-32 showed that the former distillation choice is indeed a better trader of plasticity for rigidity.

Second, we adapted the pooled output distillation losses to ViTs, and showed how the symmetric nature of its distance metric limited rigidity by penalizing the increased attention for older knowledge. We proposed an asymmetric variant of the metric to address this shortcoming. The reformulation consistently leads to not only a gain in rigidity but also on the average accuracy scores. Finally, we provided a first comprehensive evaluation of popular CL techniques adapted to ViTs with the hope to open the doors for further research in this direction. Given the inherent capability of our asymmetric loss to preserve attention A yet another interesting direction for future work could be to see the effectiveness of our asymmetric loss on multilabel CL settings.



%%%%% podnet discussion old
%Given that $\mathcal{L}_{\text{POD-spatial}}$ considers the spatial correspondence of the feature representations, extending such knowledge to ViTs is not straightforward due to the multi-head setup. During the computation of contextualized embeddings, the "spatiality" of the embeddings indeed gets distributed across several SAM heads despite being encoded along a single dimension. As a result, $\mathcal{L}_{\text{PAD-spatial}}$ would have only a first dimension resonating with the \textit{spatiality} of the inputs while the second dimension would refer to the features derived from the value tokens. We first propose employing  $\mathcal{L}_{\text{PAD-spatial}}$ to the contextualized embedding layers given their correspondence to the outputs of the CNN layers. Such a setting rather falls into our functional-based regularization category.  We then exploit the prescaled self-attention maps of ViTs and pool along both the dimensions of the map for each SAM head. This latter strategy can be classified into our \textit{attention-based} methods and forms the source for our nomenclature for ``pooled attention distillation".
